Making an Invisibility Cloak: Real World Adversarial Attacks on Object Detectors

We present a systematic study of adversarial attacks on state-of-the-art object detection frameworks. Using standard detection datasets, we train patterns that suppress the objectness scores produced by a range of commonly used detectors, and ensembles of detectors. Through extensive experiments, we benchmark the effectiveness of adversarially trained patches under both white-box and black-box settings, and quantify transferability of attacks between datasets, object classes, and detector models. Finally, we present a detailed study of physical world attacks using printed posters and wearable clothes, and rigorously quantify the performance of such attacks with different metrics.

==> patch.tex <==
%!TEX root = 1425.tex 
\begin{figure*}[h]
    \centering
    \resizebox{0.8\linewidth}{!}{
    \begin{subfigure}[b]{0.12\linewidth}
    \includegraphics[width=1.0\linewidth]{gallery/patches/R50-C4}
    \caption{C4}
    \end{subfigure}
    \begin{subfigure}[b]{0.12\linewidth}
    \includegraphics[width=1.0\linewidth]{gallery/patches/R50-C4-r}
    \caption{C4-r}
    \end{subfigure}
    \begin{subfigure}[b]{0.12\linewidth}
        \includegraphics[width=1.0\linewidth]{gallery/patches/R50-FPN}
        \caption{FPN}
    \end{subfigure}
    \begin{subfigure}[b]{0.12\linewidth}
        \includegraphics[width=1.0\linewidth]{gallery/patches/R50-FPN}
        \caption{FPN-r}
    \end{subfigure}
    \begin{subfigure}[b]{0.12\linewidth}
        \includegraphics[width=1.0\linewidth]{gallery/patches/Ens2}
        \caption{Ens2}
    \end{subfigure}
    \begin{subfigure}[b]{0.12\linewidth}
        \includegraphics[width=1.0\linewidth]{gallery/patches/Ens2-r}
        \caption{Ens2-r}
    \end{subfigure}
    \begin{subfigure}[b]{0.12\linewidth}
        \includegraphics[width=1.0\linewidth]{gallery/patches/Ens3}
        \caption{Ens3-r}     
    \end{subfigure}}
    \\
    \resizebox{0.8\linewidth}{!}{
    \begin{subfigure}[b]{0.12\linewidth}
        \includegraphics[width=1.0\linewidth]{gallery/patches/Fted}
        \caption{Fted}
    \end{subfigure}
        \begin{subfigure}[b]{0.12\linewidth}
        \includegraphics[width=1.0\linewidth]{gallery/patches/Yolov2}
        \caption{Yolov2}
        \label{fig:patch_yolov2}
    \end{subfigure}
    \begin{subfigure}[b]{0.12\linewidth}
        \includegraphics[width=1.0\linewidth]{gallery/patches/Yolov3}
        \caption{Yolov3}
    \end{subfigure}
       \begin{subfigure}[b]{0.12\linewidth}
        \includegraphics[width=1.0\linewidth]{gallery/patches/Seurat}
        \caption{Seurat}
        \label{fig:patch_seurat}
    \end{subfigure}
    \begin{subfigure}[b]{0.12\linewidth}
        \includegraphics[width=1.0\linewidth]{gallery/patches/Rand}
        \caption{Rand}
    \end{subfigure}
     \begin{subfigure}[b]{0.12\linewidth}
        \includegraphics[width=1.0\linewidth]{gallery/patches/Grey++}
        \caption{G++}
    \end{subfigure}
    \begin{subfigure}[b]{0.12\linewidth}
        \includegraphics[width=1.0\linewidth]{gallery/patches/Grey}
        \caption{Grey}
        \label{fig:patches_grey}
    \end{subfigure}}
    \caption{\textbf{Adversarial patches}, and comparisons with control patches. Here, (a)-(d) are based on R50, and G++ denotes Grey++.   }
    \label{fig:patches}
\end{figure*}

==> table_yolo_frcnn.tex <==
%!TEX root = 1425.tex 
 \begin{table*}[!t]
     \centering
     \ra{1.0}
     \resizebox{.9\linewidth}{!}{
    \small
     \begin{tabular}{@{}*{16}c@{}}
     \toprule %
      \hspace{2mm}\diagbox[width=2.25cm, height=.7cm]{Patch}{\hbox{Victim}}  & & R50-C4 & R50-C4-r & & R50-FPN & R50-FPN-r & & YOLOv2 & YOLOv2-r & & YOLOv3 & YOLOv3-r \\
     \cmidrule{1-1} \cmidrule{3-4}  \cmidrule{6-7} \cmidrule{9-10} \cmidrule{12-13}
     \textsc{R50-C4}                  &  & \cval{24.5}   & \cval{24.5}     &  & \cval{31.4}    & \cval{31.4}      &  & \cval{37.9}   & \cval{42.6}     &  & \cval{57.6}   & \cval{48.3}     \\
     \textsc{R50-C4}-r                &  & \cval{25.4}   & \cval{23.9}     &  & \cval{30.6}    & \cval{30.2}      &  & \cval{37.7}   & \cval{42.1}     &  & \cval{57.5}   & \cval{47.4}     \\
     \textsc{R50-FPN}                 &  & \cval{20.9}   & \cval{21.1}     &  & \cval{23.5}    & \cval{19.6}      &  & \cval{22.6}   & \cval{12.9}    &  & \cval{40.2}   & \cval{40.3}    \\
     \textsc{R50-FPN}-r               &  & \cval{21.5}   & \cval{21.7}     &  & \cval{25.4}   & \cval{18.8}      &  & \cval{17.6}   & \cval{11.2}     &  & \cval{37.5}  & \cval{36.9}     \\
     \cmidrule{1-1}% \cmidrule{3-4}  \cmidrule{6-7} \cmidrule{9-10} \cmidrule{12-13}
     \textsc{Yolov2}                  &  & \cval{21.1}   & \cval{19}       &  & \cval{21.5}    & \cval{21.4}      &  & \cval{10.7}   & \cval{7.5}      &  & \cval{18.1}   & \cval{25.7}     \\
     \textsc{Yolov3}                  &  & \cval{28.3}   & \cval{28.9}     &  &\cval{ 31.5}    & \cval{27.2}      &  & \cval{20}     & \cval{15.9}     &  & \cval{17.8}   & \cval{36.1}     \\
     \cmidrule{1-1} %\cmidrule{3-4}  \cmidrule{6-7} \cmidrule{9-10} \cmidrule{12-13}
     \ft            &  & \cval{25.6}   & \cval{23.9}     &  & \cval{24.2}    & \cval{24.4}      &  & \cval{18.9}   & \cval{16.4}     &  & \cval{31.6}   & \cval{28.2}     \\
     \enstwo               &  & \cval{20}     & \cval{20.3}     &  & \cval{23.2}    & \cval{19.3}      &  & \cval{17.5}  & \cval{11.3}   &  & \cval{39}    & \cval{38.8}     \\
     \enstwo-r             &  & \cval{19.7}   & \cval{20.2}     &  & \cval{23.3 }   & \cval{16.8}      &  & \cval{14.9}   & \cval{9.7 }     &  & \cval{36.3}   & \cval{34.1}     \\
     \ensthree-r             &  & \cval{21.1}   & \cval{21.4}    &  & \cval{24.2}    & \cval{17.4 }     &  & \cval{13.4}   & \cval{9.0 }       &  & \cval{29.8}   & \cval{33.6 }    \\
     \cmidrule{1-1} %\cmidrule{3-4}  \cmidrule{6-7} \cmidrule{9-10} \cmidrule{12-13}
     \textsc{Seurat}                  &  & \cval{47.9}   & \cval{52}       &  & \cval{51.6}    & \cval{52.5}      &  & \cval{43.4}   & \cval{39.5}     &  & \cval{62.6}   & \cval{57.1}     \\
     \textsc{Random}                  &  & \cval{53}     & \cval{58.2}     &  & \cval{59.8}    & \cval{59.7}      &  & \cval{52}     & \cval{52.5}     &  & \cval{70 }    & \cval{63.5}     \\
     \textsc{Grey}                    &  & \cval{45.9}   & \cval{49.6}     &  & \cval{50}      & \cval{50.8}      &  & \cval{48}     & \cval{47.1}     &  & \cval{65.6}   & \cval{57.5}     \\
     \textsc{Grey++}                  &  & \cval{46.5}   & \cval{49.8}     &  & \cval{51.4}    & \cval{52.7 }     &  & \cval{48.5}   & \cval{49.4}     &  & \cval{64.8}   & \cval{58.6}     \\
     \cmidrule{1-1} %\cmidrule{3-4}  \cmidrule{6-7} \cmidrule{9-10} \cmidrule{12-13}
     \textsc{Clean}                   &  & \cval{78.7}   & \cval{78.7}     &  & \cval{82.2}    & \cval{82.1}      &  & \cval{63.6}   & \cval{62.7}     &  & \cval{81.6}   & \cval{74.5}     \\ \hline
     \end{tabular}}
     \caption{\textbf{Impact of different patches on various detectors, measured using average precision (AP).} The left axis lists patches created by different methods, and the top axis lists different victim detectors.  Here, ``r'' denotes retrained weights instead of pretrained weights downloaded from model zoos.  %Attacks are evaluated in the digital world.
     }
     \label{tbl:digital_white}
 \end{table*}

==> voc_results.tex <==
\begin{table*}[h]
\centering
\ra{1.1}
\resizebox{1.0\linewidth}{!}{
    \begin{tabular}{@{}*{23}c@{}}
    \toprule
    \hspace{2mm}\diagbox[width=2.25cm, height=.7cm]{Patch}{\hbox{Class}} && aero & bike & bird & boat & bottle & bus  & car  & cat  & chair & cow  & table & dog  & horse & mbike & person & plant & sheep & sofa & train & tv   \\ 
    \cmidrule{1-1} \cmidrule{3-22}
    \textsc{Person} && \cval{2.0 } & \cval{14.6} & \cval{1.0 } & \cval{1.8 } & \cval{2.7 } & \cval{13.5} & \cval{10.7} & \cval{2.3 } & \cval{0.1 } & \cval{2.4 } & \cval{6.4 } & \cval{2.3 } & \cval{8.3 } & \cval{12.3} & \cval{5.5 } & \cval{0.3 } & \cval{2.2 } & \cval{1.3 } & \cval{3.8 } & \cval{12.4} \\
    \textsc{Horse}  && \cval{5.0 } & \cval{31.9} & \cval{4.7 } & \cval{4.1 } & \cval{2.5 } & \cval{26.4} & \cval{17.6} & \cval{10.6} & \cval{2.3 } & \cval{26.0} & \cval{24.7} & \cval{9.5 } & \cval{27.9} & \cval{26.6} & \cval{16.0} & \cval{7.6 } & \cval{12.4} & \cval{13.4} & \cval{13.2} & \cval{35.3} \\
    \textsc{Bus}    && \cval{3.1 } & \cval{30.6} & \cval{8.5 } & \cval{4.4 } & \cval{1.9 } & \cval{18.4} & \cval{15.6} & \cval{7.8 } & \cval{2.7 } & \cval{25.7} & \cval{39.8} & \cval{5.3 } & \cval{20.8} & \cval{20.7} & \cval{16.0} & \cval{8.9 } & \cval{12.3} & \cval{9.5 } & \cval{9.3 } & \cval{29.5} \\
    \cmidrule{1-1}
    \textsc{Grey}   && \cval{3.0 } & \cval{19.0} & \cval{6.4 } & \cval{14.6} & \cval{8.5 } & \cval{26.9} & \cval{19.6} & \cval{9.9 } & \cval{9.8 } & \cval{28.6} & \cval{24.4} & \cval{7.4 } & \cval{22.7} & \cval{15.9} & \cval{35.8} & \cval{6.1 } & \cval{18.7} & \cval{8.7 } & \cval{11.4} & \cval{61.8} \\ 
    \cmidrule{1-1}
    \textsc{Clean}  && \cval{77.5} & \cval{82.2} & \cval{76.3} & \cval{63.6} & \cval{64.5} & \cval{82.9} & \cval{86.5} & \cval{83.0} & \cval{57.2} & \cval{83.3} & \cval{66.2} & \cval{84.9} & \cval{84.5} & \cval{81.4} & \cval{83.3} & \cval{48.0} & \cval{76.7} & \cval{70.1} & \cval{80.1} & \cval{75.4} \\
    \bottomrule
    \end{tabular}}
    \caption{\textbf{Transferability of patches across classes from VOC}, measured with average precision (AP).}
    \label{tbl:attack_classes}
    \end{table*}
